Know When to Fold 'Em: Self-Assembly of Shapes by Folding in Oritatami

An oritatami system (OS) is a theoretical model of self-assembly via co-transcriptional folding. It consists of a growing chain of beads which can form bonds with each other as they are transcribed. During the transcription process, the $\delta$ most recently produced beads dynamically fold so as to maximize the number of bonds formed, self-assemblying into a shape incrementally. The parameter $\delta$ is called the delay and is related to the transcription rate in nature. This article initiates the study of shape self-assembly using oritatami. A shape is a connected set of points in the triangular lattice. We first show that oritatami systems differ fundamentally from tile-assembly systems by exhibiting a family of infinite shapes that can be tile-assembled but cannot be folded by any OS. As it is NP-hard in general to determine whether there is an OS that folds into (self-assembles) a given finite shape, we explore the folding of upscaled versions of finite shapes. We show that any shape can be folded from a constant size seed, at any scale n >= 3, by an OS with delay 1. We also show that any shape can be folded at the smaller scale 2 by an OS with unbounded delay. This leads us to investigate the influence of delay and to prove that, for all {\delta} > 2, there are shapes that can be folded (at scale 1) with delay {\delta} but not with delay {\delta}'<{\delta}. These results serve as a foundation for the study of shape-building in this new model of self-assembly, and have the potential to provide better understanding of cotranscriptional folding in biology, as well as improved abilities of experimentalists to design artificial systems that self-assemble via this complex dynamical process.

==> content-for-later.tex <==
\subsection{List of impossibility results/conjectures}




Old list:
$\forall c \in \{2.0, 2.0+, 2.5\}$:
\begin{enumerate}
    \item $\exists$ shape $s_\infty$ such that $|s_\infty| = \infty$ and $\not \exists$ OS $o_\infty$ such that $o_\infty$ self-assembles $s_\infty$ at scale factor $c$ \label{item:infinite-shape}
    
    \item $\forall$ delay factor $\delta > 0$, $\exists$ shape $s_\delta$ such that $|s_\delta| < \infty$ and $\not \exists$ OS $o_\delta$ such that $o_\delta$ self-assembles $s_\delta$ at scale factor $c$ \label{item:no-delta}
    
    %\item (MJP: just adding this one for completeness - no thoughts on whether it's true) $\forall$ bead set $b$, $\exists$ shape $s_b$ such that $|s_\delta| < \infty$ and $\not \exists$ OS $o_b$ such that $o_b$ self-assembles $s_b$ at scale factor $c$ \label{item:no-bead-set}
    
    \item $\forall$ shape $s$ such that $|s| < \infty$, $\exists$ OS $o_s$ self-assembles $s$ at scale factor $c$ \label{item:all-finite}
\end{enumerate}

The proofs of \ref{item:infinite-shape} and \ref{item:no-delta} will be based on Jacob's argument about long straight segments.

%I don't have any ideas for \ref{item:no-bead-set}.

A general construction will be needed for \ref{item:all-finite}, which can use a bead set and transcript of length equal to the number of points in the scaled shape.  We'll have to determine how to ensure that all pieces fold in the correct direction.





\subsection{Self-assembly of any finite shape with arbitrary delay factor}

\begin{theorem}\label{thm:hard-coded}
Let $S$ be an arbitrary shape such that $|S| < \infty$.  For each $c \in \{2.0, 2.0+, 2.5\}$, there exists OS $\mathcal{O}_S$ such that $\mathcal{O}_S$ self-assembles $S$ at scale factor $c$.
\end{theorem}

We prove Theorem \ref{thm:hard-coded} by splitting each scale factor into its own lemma and proving each separately.

\begin{lemma}\label{lem:hard-coded-2}
Let $S$ be an arbitrary shape such that $|S| < \infty$.  There exists OS $\mathcal{O}_S$ such that $\mathcal{O}_S$ self-assembles $S$ at scale factor $2.0$.
\end{lemma}

\begin{proof}
We prove Lemma~\ref{lem:hard-coded-2} by construction.  Therefore, assume $S$ is an arbitrary shape such that $|S| < \infty$, and let $S'$ be a $2$-scaling of $S$, produced following the algorithm for the proof of Theorem~\ref{thm:scaling}. Let $H$ be the Hamiltonian cycle (HC) through $S'$ found by that algorithm, and for $n = |S'|$ (the number of locations in $S'$), let $P = p_0, p_1, \ldots,p_{n-1}$ be an ordering of the points of $H$ such that $p_0$,$p_1$, and $p_2$ are points $6$, $1$, and $2$, respectively, (as the points of a pixel gadget are labeled in Figure~\ref{fig:point-nbrs}, i.e. NW, NE, and E) of the first pixel gadget added by the algorithm.\footnote{The only requirement for these three points is simply that they are $3$ consecutive connected points in the same pixel gadget in $H$, and by the definition of the algorithm which creates $H$, these three points are guaranteed to be such since the first pixel gadget represents the leftmost of the top points of $S$ and therefore there are no neighboring points which could cause those edges to be removed as future pixel gadgets are added.} We will break $H$ between $p_{n-1}$ and $p_0$ to form our transcript sequence. We now define OS $\mathcal{O}_{S'} = (\Sigma, \omega, \calH, \delta, \beta, \alpha, \sigma)$ such that $\mathcal{O}_{S'}$ self-assembles $S'$. The set of bead types $\Sigma$ will contain a unique bead type for each point in $H$, and thus $|\Sigma| = n$. The seed $\sigma$ will be the first three bead types in locations $p_0$, $p_1$, and $p_2$.    The transcript $w$ will be a finite transcript, with $|w| = n-3$, which enumerates the bead types $p_3,p_4,\ldots,p_{n-1}$, in the order of $P$. The delay factor $\delta$ will be $n-3$ (i.e. the full length of the transcript). The extension-length $\beta = 1$ and arity $\alpha = 4$. The rule set $\calH$ is defined by inspecting $H$ overlaid with the ordering of bead types $P$, and adding a pair of bead types to $\calH$ for every pair of adjacent beads which are not connected via the routing, therefore allowing a bond to form between every pair of adjacent beads not already connected by the routing.

\begin{figure}[htb]
\centering
\includegraphics[width=4.0in]{images/gadget-configs.pdf}
\caption{The beads of pixel gadgets in various configurations, shown with portions of routing (black) connecting some of them and bonds (red) between them.}\label{fig:gadget-configs}
\end{figure}

We now prove that $\mathcal{O}_S$ is a deterministic system whose single terminal configuration has shape $S'$.  First, it is obvious by the design of $\mathcal{O}_S$ that the beads can be placed into the shape of $S'$ by exactly tracing the HC through $S'$ with the $n$ beads corresponding to the $n$ locations in $S'$.  We call this the \emph{designed configuration} and note that $\mathcal{O}_S$, specifically the rule set $\calH$, is designed so that when the beads are laid out in this configuration, every neighboring pair of beads which is not connected by the transcript can form a bond, and furthermore, no bead can form a bond with any other bead other than those which are neighboring in this configuration.  Therefore, the designed configuration contains the maximal number of bonds which can be formed.

To complete the proof, we must simply show that there is no configuration other than the designed configuration which can contain as many bonds.  We prove this by first noting that in $S'$, there are $7$ points which form the pixel gadget corresponding to each point of $S$ (note that points other than the center may be shared by adjacent pixel gadgets), and proving the following series of claims about the beads of each pixel gadget.

Let $k = |S|$ and $0 \le i < k$, then $g_i$ is the pixel gadget of $S'$ corresponding to point $i$ of $|S|$. In the designed configuration of $\mathcal{O}_S$, there are $7$ beads which correspond to each $g_i$.

\begin{claim}\label{claim:gadget-configs}
There is exactly one configuration of the beads of each $g_i$, modulo rotation and reflection, which allows for the formation of the maximum number of bonds which can be formed among those beads, and that is the subset of the designed configuration corresponding to those beads, modulo rotation and reflection.
\end{claim}

\begin{proof}
To prove Claim \ref{claim:gadget-configs}, we first note that the bead in the center of the designed configuration of $g_i$ must be (1) connected to two other beads of $g_i$ by transcript connections (by the definition of the transcript) and, in order to form the maximum number of possible bonds, it must form bonds with the other $4$ beads of $g_i$, or (2) in the case of $g_0$ it may be connected via the transcript to only one other bead of $g_0$ due to the location where the HC was broken (to form the path of the transcript), but will then be able to form bonds with the other $5$ beads of $g_0$. In order for this single bead to have all of these connections, it must be situated in the center of a hexagon with those beads surrounding it.  This guarantees that the $7$ beads of the $g_i$ must be arranged in the shape of a pixel gadget (i.e. a hexagon) with the bead in the center matching the center bead of the designed configuration.  To prove that the $6$ beads around the perimeter are in the same relative locations as in the designed configuration (and can't be reordered), we consider the transcript routing and/or bonds between them.  Depending on the arrangement and ordering of pixel gadgets in location neighboring $g_i$, there may or may not be a connection between a pair of beads on $g_i$'s perimeter formed by the transcript.  However, for any pair that are neighbors in the designed configuration for which there is not such a connection, those two beads can form a bond. Therefore, for the transcript ordering to be maintained as well as for the maximum number of bonds to be formed, the set of all pairs of neighboring beads on the perimeter must match the set of all pairs on the perimeter of the designed configuration, which fixes the ordering of the beads (modulo rotation and reflection).  This, along with the fact that the center bead matches that of the designed configuration, proves Claim \ref{claim:gadget-configs} that the beads of $\mathcal{O}_S$ corresponding to $g_i$ must match the designed configuration, modulo rotation and reflection.
\end{proof}

\begin{claim}\label{claim:seed-orient}
The beads corresponding to the pixel gadget $g_0$ (which contains the seed), must have the same orientation as $g_0$ in $S'$.
\end{claim}

\begin{proof}
The proof of Claim \ref{claim:seed-orient} follows immediately from the fact that the placement of the first three beads of $g_0$ are fixed by the definition of the seed.  Given that $g_0$ must have the same configuration as the corresponding beads in the designed configuration (by Claim \ref{claim:gadget-configs}), which matches that portion of $S'$, the fixed location of the first $3$ beads forces its orientation, i.e. rotation and reflection, to match that of $S'$.
\end{proof}

\begin{claim}\label{claim:gadget-orients}
For each $0 \le i < k$, the beads corresponding to $g_k$ must have the same orientation as $g_k$ in $S'$.
\end{claim}

\begin{proof}
We prove Claim \ref{claim:gadget-orients} by induction on $g_i$.  Our inductive hypothesis is that, given that the beads corresponding to $g_i$ have the same orientation as $g_i$ in $S'$, then the same must hold for those of $g_{i+1}$.  Our base case is $g-0$, which holds by Claim \ref{claim:seed-orient}.  Given that the beads corresponding to $g_i$ are oriented to match $S'$, and that by definition of $H$, $g_{i+1}$ must share $2$ beads with $g_i$ and that the beads corresponding to $g_{i+1}$ must be in the configuration matching $S'$ (by Claim \ref{claim:gadget-configs}), then the only possible orientation for the beads of $g_{i+1}$ is that which matches $S'$.
\end{proof}


Finally, the proof of Lemma~\ref{lem:hard-coded-2} follows from the fact that $\mathcal{O}_S$ results in a configuration with exactly as many beads as points in $S'$ and Claims~\ref{claim:gadget-configs}-\ref{claim:gadget-orients} which prove that those beads must fold into a configuration in shape $S'$.
\end{proof}

[MJP TODO: Need to prove it's true for scale factors $2.0+$ and $2.5$, too.]

\begin{lemma}\label{lem:hard-coded-2-plus}
Let $S$ be an arbitrary shape such that $|S| < \infty$.  There exists OS $\mathcal{O}_S$ such that $\mathcal{O}_S$ self-assembles $S$ at scale factor $2.0+$.
\end{lemma}

We first show how to form a Hamiltonian cycle $H$ through $S'$, which is the shape $S$ at scale factor $2.0+$.  This is a trivial modification (and simplification) of the algorithm for scale factor $2.0$. [MJP TODO: give a sketch]

We now define $\mathcal{O}_S$ for this scale factor (which is very similar to that for scale factor $2.0$). 

Finally, we prove that $\mathcal{O}_S$ self-assembles $S'$. [MJP TODO: This is nearly identical to the proof for $2.0$.]

\begin{lemma}\label{lem:hard-coded-2.5}
Let $S$ be an arbitrary shape such that $|S| < \infty$.  There exists OS $\mathcal{O}_S$ such that $\mathcal{O}_S$ self-assembles $S$ at scale factor $2.5$.
\end{lemma}

[MJP TODO: This is extremely similar to scale factor $2.0+$.]


==> definitions-formal.tex <==
\section{Formal Definitions for The Oritatami Model and Shapes}\label{sec:definitions-formal}

We now provide formal definitions relating to the oritatami model. These definitions are required in order to give rigorous proofs of our results (especially the impossibility results in Section~\ref{sec:sdw}).

\subsection{Graphs and functions}

We now define the triangular grid graph and other definitions related to graphs which will be useful in later definitions.

\begin{definition}
We say that a \emph{graph $G=(V, E)$ is induced by a set $S \in \mathbb{R}^2$} if the vertices of $G$ are points in $S$, and the edges of $G$ connect the vertices that at distance $1$; i.e., $V=S$, $E=\{\{i,j\} \mid i, j \in S,\ |i-j|=1\}$.
%\todo{TAR: This was taken from Demaine's paper on hamiltonian paths in grid graphs}
\end{definition}

We now give the definitions of the triangular grid graph referred to in this paper.

\begin{definition}
Let $\mathbb{Z}_{\Delta}$ be the set of points in $\mathbb{R}^2$ given by the Cartesian coordinates of end points of vectors in the vector space generated by $\langle 1,0 \rangle$ and $\langle \frac{1}{2}, \frac{\sqrt{3}}{2}\rangle$.  The \emph{triangular grid graph} is the plane graph induced by a subset of vertices of $\mathbb{Z}_{\Delta}$.  Let $E_{\Delta}$ denote the set of edges of the graph induced by $\mathbb{Z}_{\Delta}$, let $\mathbb{T} = (\mathbb{Z}_{\Delta}, E_{\Delta})$, and let et $U_{\Delta}$ be the set of unit vectors defined by $U_{\Delta}= \{ \vec{m} - \vec{n} \mid \{ \vec{m}, \vec{n} \} \in E_{\Delta} \}$.  Note $|U_{\Delta}|=6$.
\end{definition}

Because an oritatami system models the folding of a sequence of beads by paths in $\mathbb{T}$, we now define paths in a graph $G$.

\begin{definition}
Let $G=(V, E)$ be a graph and let $k\in N$\footnote{We follow the convention that $0\in \N$.}.  A \emph{directed path in G} is a sequence $P=(p_i)_{i=0}^k$ in $V$, of pairwise-distinct vertices in $V$ such that $\{p_i, p_{i+1}\} \in E$ for all $1 \leq i \leq k$.  We call $k$ the length of $P$.
\end{definition}

Let $a = (a_i)_{i=1}^k$ be a sequence of points in $\mathbb{T}$.  We denote the $i^{th}$ element of $a$ by $a(i)$; that is, $a(i)=a_i$. Similarly, we define $range(a)$ to be the set of points of $a$; that is, $range(a) = \cup_{i=1}^k a_i $.

For $G = (E,V)$ and $G' = (E',V')$ graphs, to denote that a graph $G'$ is a subgraph of $G$, we write $G' \sqsubseteq G$. When $G'$ and $G$ are weighted graphs with weights given by functions from $E$ to $\mathbb{N}$ which we call $w$ and $w'$ respectively, we use $G' \sqsubseteq G$ to denote that $G'$ is a subgraph of $G$ and $w(e) = w'(e)$ for all $e\in E'$.


\subsection{Bead types and rule sets}

We now define the fundamental concepts that constitute an oritatami system: bead types, bond rules, beads, and bonds.

\begin{definition}[Bead Type]
A \emph{set of bead types} is a finite alphabet $\Sigma$.  We refer to a member of $\Sigma$ as a bead type.  For $a \in \Sigma$, we say that $a$ is a bead of type $a$ or we refer to it as an $a$-bead.
\end{definition}

By $\Sigma^*$ and $\Sigma^{\omega}$, we denote the set of finite sequences of bead types in $\Sigma$ and that of one-way infinite sequences of bead types in $\Sigma$, respectively.  A sequence $w \in \Sigma^* \cup \Sigma^\omega$ can be written as $w=b_1b_2 \dots $ for $b_i \in \Sigma$.  If $w$ is finite, there exists an integer $n \geq 0$ satisfying $w = b_1b_2 \dots b_n$; such $n$ is called the length of $w$ and is denoted by $|w|$.  The sequence of length $0$ is denoted by $\lambda$.  For $|w| \geq i, j, \geq 1$, the subsequence of $w$ ranging from the $i^{th}$ bead type to the $j^{th}$ bead is denoted by $w[i \dots j]$; that is $w[i \dots j] = b_ib_{i+1} \dots b_j$.  If $i > j$, then $w[i \dots j]= \lambda$.  This notation is simplified to $w[i]$ when $i=j$, referring to the $i^{th}$ bead type of $w$.  For $k \in \mathbb{Z}^+$, $w[1 \dots k]$ is called a prefix of $w$ and it is said to be proper if $w$ is infinite or $k < |w|$. We denote the concatenation of two sequences $A$ and $B$ by $AB$, and in the case that $B=b$ is just a sequence with a single element, we write $Ab$ to denote the concatenation.  We denote the number of elements in $A$ by $|A|$ when $A$ is a finite sequence and define $|A|$ to be $\infty$ otherwise.

\begin{definition}[Bond Rules]
 Let $\Sigma$ be a set of bead types.  A \emph{rule set} $\mathcal{H} \subseteq \Sigma \times \Sigma$ is a symmetric relation over the set of pairs of bead types\footnote{that is, for all bead types $a, b \in \Sigma$, $(a, b) \in \mathcal{H}$ implies $(b,a) \in \mathcal{H}$}.  We refer to elements of $\mathcal{H}$ as \emph{bond rules}.
 \end{definition}

We now give a formal definition of a bead and a bond between two beads.

\begin{definition}[Bead and Bond]
 Let $\Sigma$ be a set of bead types.  A \emph{bead} is an ordered pair $(p,t)$ where $p\in \mathbb{T}$ and $t\in \Sigma$.
 Additionally, for two beads $b, b' \in \mathbb{Z}_{\Delta} \times \Sigma$, a \emph{bond} between $b$ and $b'$ is an ordered pair $(b,b')$.
\end{definition}

An oritatami system models the folding sequences of beads into complexes called configurations which we define in the next section.

\subsection{Configurations and conformations}
Configurations are a formalization of the structures that oritatami systems fold. Informally, an oritatami systems is intended to capture the folding of a ``string of beads'' (defined by a sequence of symbols from an alphabet $\Sigma$) to yield complex structures. A bead belonging to such a string of beads may attract another bead in the string of beads and such attractions (defined in a rule set) determine the structures that result from the folding of the string of beads. Definition~\ref{def:routing} formally captures the notion of a folded ``string of beads'' which we formally refer to as a \emph{routing}. Note that the definition of a routing does not capture anything about bead interactions.

\begin{definition}[Routing]\label{def:routing}
Let $\Sigma$ be a set of bead types.  Also, let $w \in \Sigma^* \cup \Sigma^\omega$, and let $P$ be a directed path of $\mathbb{T}$ of length $|w|$.  Moreover, let $R = \{b_i\}_{i=1}^{|w|}$ be a sequence of beads over $\mathbb{Z}_{\Delta} \times \Sigma$
 and let $p_i\in \mathbb{Z}_{\Delta}$ and $w_i\in \Sigma$ be such that $b_i=(p_i, w_i)$. Then, $R$ is a \emph{routing of $w$ along $P$} if
$p_i = P[i]$ and $w_i = w[i]$ for all $i$ such that $1\leq i \leq |w|$.  We denote that $R$ is a routing of $w$ along $P$ by writing $R=(P, w)$.  When $w$ and $P$ are clear from context, we simply refer to $R$ as a routing.
\end{definition}

We can now formally define a configuration of beads. In the following definition, let $(\Sigma \times \mathbb{Z}_{\Delta})^{\mathbb{N}}$ denote the set of sequences in $\Sigma \times \mathbb{Z}_{\Delta}$.

\begin{definition}[Configuration]
Let $\Sigma$ be a set of bead types, let $w \in \Sigma^* \cup \Sigma^\omega$, let $P$ be a directed path of length $|w|$.  A \emph{configuration} $C$ is a pair $(R, H) \in (\Sigma \times \mathbb{Z}_{\Delta})^{\mathbb{N}} \times \mathcal{P}([1, |w|] \times [1,|w|])$ where $R = (P, w)$ is the routing of $w$ along $P$ and $H \subset \{(i,j) \mid 1 \leq i, \ i+2 \leq j, \ P(i)-P(j) \in U_{\Delta} \}$.  We call $H$ the \emph{set of bonds of the configuration $C$}.
\end{definition}

An \emph{empty configuration} is defined to be any configuration $(P,w,H)$ where $P = H = \emptyset$.
For a configuration $C=(P,w,H)$, the \emph{number of bonds} in $C$, denoted $\mathcal{B}(C)$, is defined by $\mathcal{B}(C)=|H|$. By a slight abuse of notation, we will also write $C=(P,w,H)$ as opposed to $C=(R, H)$ where $R=(P,w)$.  We call a configuration $C=(P,w,H)$ finite if $|P|$ is finite.  Otherwise we call $C$ an infinite configuration.  The domain of a configuration $C=(P,w,H)$ written $dom(C)$ is defined by $dom(C) = range(P)$. (Note that $range(P)$ is the set of points of $\Z_\Delta$ belonging to the path $P$.)

We now formally define an interaction graph of a configuration $C=(P,w,H)$.  Intuitively, this is a triangular grid graph consisting of nodes which are in the path $P$ such that there is a 0-weight edge between nodes if they are ``linked'' by the path and a 1-weight edge if they share a bond in $H$.  Note that this will be convenient because the sum of the weights of the edges will tell us how many bonds are in the structure and the path of 0-weight edges corresponds to how a sequence of beads is folded in a configuration.

\begin{definition}[Interaction Graph]
Let $\Sigma$ be a set of bead types, let $w \in \Sigma^* \cup \Sigma^\omega$, let $P$ be a directed path of length $|w|$.  Furthermore, let $C=(P, w, H)$ be a configuration.  The \emph{interaction graph of configuration $C$}, denoted $G_C$, is the edge-weighted graph $G_C = (V, E)$ given by $V=range(P)$, and $\{\vec{m}, \vec{n} \} \in E$ if and only if
\begin{enumerate}
  \item there exists $i, j \in [1, |w|]$ such that $P(i) = \vec{m}$ and $P(j) = \vec{n}$ and $|i-j|=1$ in which case the weight of the edge$\{\vec{m}, \vec{n}\}$ is $0$, or
  \item there exists $i, j \in [1, |w|]$ such that $P(i) = \vec{m}$ and $P(j) = \vec{n}$ and $\{i,j\} \in H$ in which case the weight of the edge $\{\vec{m}, \vec{n}\} = 1$.
\end{enumerate}
\end{definition}

Often times the exact embedding of a structure in the plane is of no importance.  We now define a conformation which can be thought of as the set of all rigid transformations of a configuration.  We say two configurations are the same conformation if they can be rigidly transformed into one another.

\begin{definition}[Conformation]
Let $(P_1, w_1, H_1)$ and $(P_2, w_2, H_2)$ be configurations.  We say $(P_1, w_1, H_1)$ and $(P_2, w_2, H_2)$ are \emph{congruent} provided that $w_1=w_2$, $H_1 = H_2$, and there exists an isometry $T: \mathbb{R}^2 \rightarrow \mathbb{R}^2$ such that $P_1(i) = T(P_2(i))$ for all $i \in [1, |w|]$.  The set of all configurations congruent to the configuration $(P, w, H)$ is called the \emph{conformation} of the configuration and denoted by $[(P, w, H)]$.
\end{definition}

For a rule set $\mathcal{H}$ over an alphabet $\Sigma$, a configuration $C$ is $\mathcal{H}$-valid provided that the bonds between the bead types in $C$, which is given by the set $H$, correspond to bond rules in $\mathcal{H}$.  The following is a more formal definition of this notion.

\begin{definition}[$\mathcal{H}$-valid]
Let $C=(P,w,H)$ be a configuration.  We say a bond $(i,j) \in H$ is \emph{valid with respect to $\mathcal{H}$} or simply \emph{$\mathcal{H}$-valid} if $(w[i], w[j]) \in \mathcal{H}$.  The configuration $C$ is $\mathcal{H}$-valid provided that all elements of $H$ are $\mathcal{H}$-valid. When $\calH$ is clear from context we use the term \emph{valid} for $\calH$-valid.
\end{definition}

The arity of a configuration $C=(P,w,H)$ is the maximum number of bonds in $H$ that a bead can have with its neighbors.  For example, an arity $1$ system is one with the restriction that a single bead can only bind one other bead.  Since a single bead in the triangular grid can have at most six neighbors the maximum arity of any configuration is bounded by $6$. In fact, as everybead in a configuration belongs to the path $P$ and bonds to not exist between consecutive points in the path $P$ by definition, the maximum arity of any configuration is bounded by $5$.

In the following definition, we use the convention that if $k \in \mathbb{N}$ is finite $[1, k] = \{i \mid i \in \mathbb{N} \text{ and } 1 \leq i \leq k \}$ and if $k = \infty$, $[1,k] = \mathbb{N}\setminus \{0\}$.

\begin{definition}[Arity]
Let $C=(P,w,H)$ be a configuration, and let $\alpha \in [1,5]$.  We say that $C$ has \emph{arity} $\alpha$ provided that for any $i \in [1, |w|]$, $|\{(i, k) \mid (i,k) \in H \}| \leq \alpha$.
\end{definition}

We define the arity of a configuration $C$, denoted $arity(C)$, as $arity(C) = min(\{\alpha | C \text{ has arity } \alpha\})$.
Next we define the ``subconfiguration'' relation between two configurations. Intuitively, a configuration $C'$ is a subconfiguration of $C$ provided that $C'$ is contained in $C$.

\begin{definition}[Subconfiguration]
Let $C' = (P', w', H')$ and $C = (P, w, H)$ be configurations.  We say that $C'$ is a subconfiguration of $C$ and write $C' \sqsubseteq C$ provided that $G_{C'} \sqsubseteq G_C$.
\end{definition}

\subsection{Elongations}

We now focus on elongations of configurations.  Intuitively, configurations in oritatami system ``grow'' by ``elongating'' (i.e. added beads to a path) the routing of such a configuration to obtain a set of possibly many elongated configurations. Then an elongated configurations which maximizes the number of bonds is considered and some fixed number (given as a parameter of the system) beads ``stabilize'' to form a configuration that contains the configuration from which it grew.  We now provide definitions of the machinery which allows us to formally describe this process.

Intuitively, an elongation of a configuration $C = (P, w, H)$ by a bead $b$ is a configuration where the path has been extended by another point and $b$ is placed at that point.  The bonds of an elongation of $C$ must contain all elements of $H$ and may have additional bonds which contain the newly added bead.

\begin{definition}[Elongation]\label{def:elongation}
Let $\Sigma$ be a set of bead types, let $w_1, w_2 \in \Sigma^* \cup \Sigma^w$, let $P_1$ be a directed path of length $|w|$. For a finite configuration $C_1= (P_1, w_1, H_1)$, another finite configuration $C_2 = (P_2, w_2, H_2)$ is an \emph{elongation} of $C_1$ by a bead $b \in \Sigma$, written as $C_1 \xrightarrow[b]{} C_2$ provided that
\begin{enumerate}
  \item $P_2 = P_1p$ for some $p \in \mathbb{Z}_{\Delta}$,
  \item $w_2 = w_1b$, and
  \item $H_1 = \{(i,j) | (i,j) \in H_2 \text{ and } 1 \leq i,j \leq |w_1|\}$.
\end{enumerate}
The definition of elongation is recursively extended to the elongation by $w \in \Sigma^*$.  For any configuration $C$, $C \xrightarrow[\lambda]{} C$; and for $w=w_1w_2 \dots w_n \in \Sigma^*$, a configuration $C_2$ is an elongation of $C_1$ by $w$ if there is a configuration $C'$ such that $C_1 \xrightarrow[w[1 \dots n-1\text{]}]{} C'$ and $C' \xrightarrow[w_n]{} C_2$.
\end{definition}

In Definition~\ref{def:elongation}, for a rule set $\mathcal{H}$, if $C_1$ and $C_2$ are both $\mathcal{H}$-valid configurations, we say that $C_2$ is an \emph{$\mathcal{H}$-valid elongation of} $C_1$, and we use $C_1 \xrightarrow[w[1 \dots n-1\text{]}]{\mathcal{H}} C_2$ to denote this relation.   Moreover, for $\alpha \in [1,5]$, if $arity(C_2) \leq \alpha$, we say that $C_2$ is an elongation of $C_1$ \emph{with arity $\alpha$}\footnote{Note that this implies that $arity(C_1)\leq \alpha$.}.

Note that there is a straight forward extension of the definition of elongation to conformations.

\begin{definition}
For confirmations $S$ and $S'$, we say that $S'$ is an elongation of $S$ provided that there exists a configuration $C'$ in $S'$ and a configuration $C$ in $S$ such that $C'$ is an elongation of $C$.
\end{definition}

During the folding process of an oritatami system the next bead to be stabilized in the system depends on the elongation of the current configuration which makes the most bonds.  In order to discuss all elongations of a configuration, we now define the set of $\mathcal{H}$-valid elongations of $C$ by $t$ with arity $\alpha$ where $t$ is a sequence of bead types.


\begin{definition}[$\calH$-valid Elongations]
Let $\Sigma$ be a set of bead types, $w \in \Sigma^* \cup \Sigma^\omega$, $t \in \Sigma^*$, $\alpha \in [1,5]$, and $\mathcal{H}$ be a rule set over $\Sigma$.  Furthermore, let $C=(P,w,H)$ be an $\calH$-valid configuration.  The set of \emph{$\calH$-valid elongations of $C$ by $t$ with arity $\alpha$}, denoted $\calP_{\calH, \alpha}^t(C)$, is defined by $\calP_{\calH, \alpha}^t(C)=\{C' | C \xrightarrow[t]{\calH} C' \text{ and } arity(C') \leq \alpha \}$. Let $p(t)$ be the set of prefixes of $t$. The set of \emph{$\calH$-valid elongations by prefixes of $t$ with arity $\alpha$}, denoted $\calP_{\calH, \alpha}^{\leq t}(C)$, is defined by $\calP_{\calH, \alpha}^{\leq t}(C)= \cup_{t' \in p(t)} \calP_{\calH, \alpha}^{t'}(C)$.
\end{definition}

Let $C'$ be an elongation of $C$.  The \emph{length of the elongation} of $C$ by $C'$, denoted $L(C', C)$, is $L(C', C) = |dom(C') \setminus dom(C)|$.

To formally discuss the elongations of a configuration which contain the most bonds, we define the set of ``favorable elongations''.  Let $s\in \Sigma^*$ be some bead sequence.  The favorable elongations of a configuration $C$ by $s$ are those which are in the set of elongations of $C$ by $s$ and form the most bonds out of all other configurations in that set. We consider elongations by prefixes of $s$ as opposed to only considering elongations by $s$ due to the fact that there may be a ``crevice'' in a configuration which is such that only less than $|s|$ number of beads can fit into the ``crevice'' in a way that creates a large number of bonds.  This is the configuration which creates the most number of bonds, but this configuration would be missed if we only considered elongations by $s$.  Assuming this is the most ``favorable'' configuration, an oritatami system is defined in such a way that the shortened elongation would be considered the favorable configuration.

\begin{definition}[Favorable Elongations]
Let $\Sigma$ be a set of bead types, $s, w \in \Sigma^*$, $\alpha \in [1,5]$, $\delta\in \N$, and $\mathcal{H}$ be a rule set over $\Sigma$.  Furthermore, set $\delta = |s|$, and let $C=(P, w ,H)$ be a finite configuration.

A configuration $C_f$ is called a \emph{favorable $\alpha$-$\delta$-elongation of $C$ by $s$ under rule set $\calH$} provided that
\begin{enumerate}
\item $C_f \in \calP_{\calH, \alpha}^{\leq s}(C)$, and
\item $\forall C' \in \calP_{\calH, \alpha}^{\leq s'}(C)$ and $s' \in \Sigma^*$ such that $|s'| = \delta$, $\calB(C') \leq \calB(C_f)$.
\end{enumerate}
We denote the set of favorable $\alpha$-$\delta$-elongations of $C$ by $s$ under $\calH$ by ${\calF}_{\calH, \alpha}^{ s}(C)$. When $\alpha$ and $\delta$ are clear from context, simply refer to favorable $\alpha$-$\delta$-elongations as \emph{favorable elongations}.
\end{definition}

Once an oritatami system ``detects'' a next most favorable configuration $C_f$, it doesn't blindly place beads until $C_f$ assembles.  But rather, for a fixed integer parameter of the oritatami system which we call $\beta$, it only stabilizes the ``next $\beta$ beads'' based on $C_f$ and then it repeats the process of finding the next favorable configuration (which doesn't necessarily need to agree with $C_f$). To formally define the notion of ``stabilizing the next $\beta$ beads'' we have the following definition of an \emph{L-projection}.

\begin{definition}[L-projection]
Let $\Sigma$ be a set of bead types, $w = b_1b_2 \dots b_n \in \Sigma^*$ be a sequence of $n$ bead types, and let $P=p_1p_2 \dots p_n$ be a directed path in $\mathbb{T}$.  Furthermore, let $C=(P,w,H)$ and $L \in \mathbb{N}$ such that $L \leq n$.  The $L$-projection of $C$, denoted $\rho_{L}(C)$, is the configuration $\rho_{L}(C) = (P', w', H')$ such that
\begin{enumerate}
  \item $|P'| = n - L$ and $P'(i) = P(i)$ for all $i \in [1, n - L]$,
  \item $w' = b_1b_2 \dots b_{n-L}$, and
  \item $H' = H \setminus \{ (i,j) \mid (i,j) \in H \text{ and } i > n-L \text{ or } j > n-L \}$.
\end{enumerate}

\noindent When $L > n$, $\rho_L(C)$ is defined to be the empty configuration.

\end{definition}


\subsection{Configuration sequences}

%Looking to the definition of the abstract tile assembly model (aTAM) in [TAR: cite Scott/Jack] as inspiration, we now define the equivalent of an assembly sequence in the aTAM.  Assembly sequences are often a cornerstone in impossibility results in the aTAM.  By showing that the assembly sequence is restricted in some way, we can limit the final products the adversary is able to assemble.  The fundamental importance of assembly sequences in the aTAM lead us to believe they will be essential in the oritatami model.

%Unlike the aTAM where it makes sense to only consider the sequence of intermediary assemblies leading to the final assembly, in oritatami we must consider two types of ``assembly'' sequences.  The most obvious ``assembly'' sequence to consider in oritatami is the sequence of intermediary configurations.  These are the configurations where all the beads are ``stabilized'' (that is, they are fixed in that position for the remainder of the ``assembly'' sequence).  We call this the foldable sequence.

%In order to actually obtain the foldable sequence of a system, we must consider a less obvious ``assembly'' sequence which we call the $\alpha$-$\delta$-favorable sequence over a bead type sequence $w$.  The favorable sequence begins with some configuration which we call $C_0$.  The next configuration $C_1$ is then a favorable $\alpha$-$\delta$-elongation of $C_0$.  To obtain $C_i$ for $i > 1$, take the $\delta$-projection of the previous configuration (which removes the $\delta-1$ last beads in the previous configuration) and then find a favorable $\alpha$-$\delta$-elongation of the $\delta$-projection.  We refer to the last $\delta-1$ beads of a configuration in the favorable sequence as the nascent portion of the configuration since these are intuitively the beads which are not yet stabilized but assist in determining where the next bead should be stabilized.

%Note that the elements of a favorable sequence are not necessarily subconfigurations of one another since a bead in the nascent portion can change positions multiple times before it is ``stabilized''.  A favorable sequence of an oritatami system completely defines the foldable configurations of the system.  To obtain the foldable configurations of the system, simply take the $\delta$-projection of the $i^{th}$ favorable configuration for $i>0$.  It should be noted that a favorable configuration does not necessarily appear at some point as a foldable configuration.\todo{TAR: Maybe show an example of why this is the case.}

In the oritatami model, the process of folding a sequence of beads is captured by sequences of configurations. In particular, we consider special sequences of configurations called \emph{foldable sequences}. Let $\Sigma$ be a set of bead type, and let $w=b_1b_2 \dots \in \Sigma^*$ and $b_i\in \Sigma$ for all $1\leq i\leq |w|$.  In the following definition, we use the convention that for $i,k\in \N$, if $k > |w|$ and $i \leq |w|$, then $w[i \dots k] = w[i \dots |w|]$.

\begin{definition}[Foldable Sequence]\label{def:foldable-sequence}
Let $\Sigma$ be a set of bead types, and let $w \in \Sigma^* \cup \Sigma^\omega$.  Also, let $C_0 = (P_0, w_0, H_0)$ be an $\calH$-valid configuration with $w_0 \in \Sigma^*$.  An \emph{$\calH$-valid $\alpha$-$\beta$-$\delta$-foldable sequence over $w$} is a sequence $\vec{C} = (C_i \mid 0 \leq i \leq k)$ in $\calP_{\calH, \alpha}^{\leq w}(C_0)$ where $k \in \mathbb{Z}^+ \cup \{ \infty \}$ and for each $i \in [1, k]$, there exists $C'_i \in \calF_{\calH, \alpha}^{\leq w[i\dots i+\delta-1]}(C_{i-1})$ such that
\begin{enumerate}
  \item $L_i = L(C'_i, C_{i-1}) \geq 1$, and
  \item $C_i = \rho_{L_i + \beta - 1}(C'_i)$.
\end{enumerate}
\end{definition}

Let $\vec{C} = (C_i)$ be an $\calH$-valid $\alpha$-$\beta$-$\delta$-foldable sequence over $w$.  For $C'_i$ given in Definition~\ref{def:foldable-sequence}, let $R_i$ be the routing of $C'_i$.  We refer to the set of beads belonging to $C'_i$ that do not belong to $C_i$ as \emph{nascent} beads. If a bead is not nascent, we call it \emph{stabilized}.

The following lemma is a formalization of the idea that the configurations in a foldable sequence are subconfigurations of proceeding configurations.  This lemma is necessary to ensure that the result of a foldable sequence exists and is well-defined. We leave the proof as an exercise.

\begin{lemma}
Let $\vec{C}_{\rho} = (C_i^{\rho})_{i=0}^k$ be an $\calH$-valid $\alpha$-$\beta$-$\delta$-foldable sequence over $w$.  Then for $i \in [0, k]$, $G_{C_{i-1}^{\rho}} \sqsubseteq G_{C_i^{\rho}}$.
\end{lemma}

The result of a foldable sequence is a configuration which can be thought of as the final product of the sequence.  In the case that a foldable sequence is finite, the result is the last configuration in the sequence.  In the case that a foldable sequence is infinite, the result is defined so that all the configurations of the sequence are subconfigurations of the result and the result contains a bead if it belongs to some configuration in the sequence.

\begin{definition}[Result of Foldable Sequence]
Let $k\in \N$ and let $\vec{C} = (C_i)_{i=0}^k$ be an $\calH$-valid $\alpha$-$\beta$-$\delta$-foldable sequence over $w$. For each $i$ ranging from $0$ to $k$, let $H_i$ be the set of bonds of $C_i$. The \emph{result} of $\vec{C}$ is the unique configuration $C$, denoted by $res(\vec{C})$, satisfying $dom(C) = \cup_{i\in [0,k]} dom(C_i)$ with set of bonds $H_{C} = \cup_{i\in [0,k]} H_i$.
\end{definition}

We now define some convenient terminology and notation.
%
Recall that in this paper we use the convention that $w$ is a prefix of itself.  %The set of $\mathcal{H}$-valid configurations over prefixes of $w$ contains all $\mathcal{H}$-valid configurations where the transcript of the configuration is a prefix of $w$.  Note that for an oritatami system which has a transcript of $w$ all valid configurations of the system will reside in this set.

\begin{notation}
Let $\Sigma$ be a set of bead types, let $w \in \Sigma^* \cup \Sigma^\omega$ and let $\mathcal{H}$ be a rule set over $\Sigma$.

\begin{itemize}
\item $\mathcal{A}_{\mathcal{H}}^w$ denotes the set of $\mathcal{H}$-valid configurations over $w$.

\item Let $p(w)$ be the set of prefixes of $w$.  $\mathcal{A}_{\mathcal{H}}^{\leq w}$ denotes the set of $\mathcal{H}$-valid configurations over prefixes of $w$. In other words, $\mathcal{A}_{\mathcal{H}}^{\leq w} = \cup_{w' \in p(w)} \mathcal{A}_{\mathcal{H}}^{w'}$.

\item $\mathcal{A}_{\mathcal{H}, \alpha}^{\leq w}$ denotes the set of $\mathcal{H}$-valid configurations over prefixes of $w$ with arity $\alpha$.
\end{itemize}

Let $C, C' \in \calA_{\calH, \alpha}^{\leq w}.$
\begin{itemize}
  \item An $\calH$-valid $\alpha$-$\beta$-$\delta$-foldable sequence over $w$ from $C$ to $C'$ is an $\calH$-valid $\alpha$-$\beta$-$\delta$-foldable sequence over $w$ $\vec{C}=(C_i)_{i=0}^k$ such that $C_0=C$ and $res(\vec{C}) = C'$.
  \item We write $C \xrightarrow[\alpha, \beta, \delta]{\calH, w} C'$ to indicate that there exists an $\calH$-valid $\alpha$-$\beta$-$\delta$-foldable sequence over $w$ from $C$ to $C'$.
\end{itemize}

\end{notation}

Given two $\calH$-valid configurations $C$ and $C'$, note that there does not necessarily exist a foldable sequence from $C$ to $C'$.

The following theorem will allow us to define a terminal configuration (which we intuitively think of as being a final product of a system) as a maximal element of the poset $(\calA_{\calH, \alpha}^{\leq w}, \xrightarrow[\alpha, \beta, \delta]{\calH, w})$. The proof of Theorem~\ref{thm:poset} is straightforward.

\begin{theorem}\label{thm:poset}
The binary relation $\xrightarrow[\alpha, \beta, \delta]{\calH, w}$ is a partial ordering of $\calA_{\calH, \alpha}^{\leq w}$.
\end{theorem}

We now define a terminal configuration based on the partial ordering $\xrightarrow[\alpha, \beta, \delta]{\calH, w}$.

\begin{definition}[Terminal Configuration]
A configuration $C \in \calA_{\calH, \alpha}^{\leq w}$ is terminal if it is a $\xrightarrow[\alpha, \delta]{\calH, w}$-maximal element of $\calA_{\calH, \alpha}^{\leq w}$.
\end{definition}

The next lemma will allow us to say that every oritatami system has a terminal configuration. We leave the proof as an exercise.

\begin{lemma}
For each $C \in \calA_{\calH, \alpha}^{\leq w}$, there exists $C' \in \calA_{\calH, \alpha}^{\leq w}$ such that $C \xrightarrow[\alpha, \beta, \delta]{\calH, w} C'$ and $C'$ is terminal.
\end{lemma}

\subsection{Oritatami systems}
We now formally define oritatami system.

\begin{definition}
An \emph{oritatami system (OS)} is a 7-tuple $\Xi = (\Sigma, w, \calH, \delta, \beta, \alpha, \sigma)$ where
\begin{itemize}
  \item $\Sigma$ is a set of bead types,
  \item $w \in \Sigma^* \cup \Sigma^\omega$ is finite or infinite periodic,
  \item $\calH$ is a rule set over $\Sigma$,
  \item $\delta \in \mathbb{N}$ is the \emph{delay},
  \item $\beta \in \mathbb{N}$ is the \emph{\extlen},
  \item $\alpha \in [1,5]$ is the \emph{arity}, and
  \item $\sigma = (P_{\sigma}, w_{\sigma}, H_{\sigma})$ where $w_{\sigma} \in \Sigma^*$ is an $\calH$-valid configuration we call the \emph{seed}.
\end{itemize}
\end{definition}

For $\Xi$ defined above, we call $w$ the \emph{transcript} of $\Xi$.

\begin{notation}
Let $\Xi = (\Sigma, w, \calH, \delta, \beta, \alpha, \sigma)$ be an OS.
\begin{enumerate}
  \item The set of  foldable configurations by $\Xi$ is $\prodasm{\Xi} = \{ C \in \calA_{\calH, \alpha}^{\leq w} \mid \sigma \xrightarrow[\alpha, \beta, \delta]{\calH, w} C \}.$
  \item The set of terminal configurations produced by $\Xi$ is $\termasm{\Xi} = \{ C \in \prodasm{\Xi} \text{ and } C \text{ is terminal} \}$.
\end{enumerate}
\end{notation}

\begin{lemma}
Let $\Xi = (\Sigma, w, \calH, \delta, \alpha, \sigma)$ be an OS, and let $C \in \prodasm{\Xi}$.  Then there is an valid foldable sequence over $w$, say $\vec{C}=(C_i)_{i=0}^k$, such that $C_0 = \sigma$ and $res(\vec{C})=C$.
\end{lemma}

Finally, an OS $\Xi$ is said to be \emph{deterministic} if $|\termasm{\Xi}| = 1$.


\subsection{Shapes and scaling}\label{sec:shape-defs}

Denote the points in $R^2$ that correspond to vertices of $\calT$ by $\Z^2_{\Delta}$.
%
We say that two points $p$ and $q$ in $\Z^2_{\Delta}$ are \emph{path-connected} if there exists a sequence of points $\{p_i\}_{i=1}^n$ over $\Z^2_{\Delta}$ where $n\in\N$ starting with $p_1 = p$ and ending with $p_n = q$ such that $p_i$ is adjacent to $p_{i+1}$ for all $i$ with $1\leq i \leq n - 1$. We say that a set of points $S$ in $\Z^2_{\Delta}$ is \emph{connected} if for any two points $p$ and $q$ in $S$, $p$ and $q$ are path-connected. A \emph{shape} $S$ is a set of connected points in $\Z^2_{\Delta}$.
%
Given an OS system $\Xi$ and a shape $S$, we say that $\Xi$ \emph{folds} (or ``self-assembles'') $S$ if for any terminal configuration $C$ of $\Xi$, the set of points defined by the locations in $\Z^2_{\Delta}$ of beads of the routing $R$ of $C$ is equal to $S$. In other words, $\Xi$ folds $S$ if every terminal assembly of $\Xi$ contains a bead at a location if and only if this location is in $S$.

Now, let $n$ be in $\N$ and let $\vec{0}$ denote the origin in $\Z^2_{\Delta}$ and let $S$ be a finite connected shape in $\Z^2_{\Delta}$. Without loss of generality, we assume that $\vec{0}$ is contained in $S$, for otherwise $S$ can be translated so that the translated $S$ contains $\vec{0}$ and then translated back to give a scaling of $S$. Now, define $Hex_n$ to be the hexagon of points in $\Z^2_{\Delta}$ equal to the set $\{ \vec{v} \in \Z^2_{\Delta}  |  \d(\vec{0}, \vec{v}) < n \}$.
%

The two methods of scaling that we define are called the \emph{$n$-scaling} of $S$ and the \emph{offset $n$-scaling} of $S$. For both methods of scaling, we refer to $n$ as the \emph{scale factor}.
To define both of the methods of scaling a shape, we define two linear transformation of $\mathbb{R}^2$ (one for each scaling method). We then apply such a transformation to $S$ to obtain a set $S'$. We then obtain a scaling of $S$ by replacing a point $\vec{p}$ of $S'$ by points of $Hex_n$ translated so that the center of $Hex_n$ is $\vec{p}$.

Specifically, to define the $n$-scaling of $S$ we let $L_1$ be the linear transformation of $\mathbb{R}^2$ which maps $(1,0)$ to $\left( \frac{3(n-1)}{2}, \frac{\sqrt{3}(n-1)}{2} \right)$ and maps $\left(\frac{1}{2},\frac{\sqrt{3}}{2}\right)$ to $\left( 0, \sqrt{3}(n-1) \right)$. Then, let $S' = L_1(S)$.  Finally, the $n$-scaling of $S$ is the union over all $\vec{p}$ in $S'$ of sets of points $Hex_n + \vec{p}= \{\vec{v}\in R^2 | \vec{v} = \vec{h} + \vec{p} \text{ for some } \vec{h}\in Hex_n \}$.  One can observe that the points of $S'$ is a subset of $\Z^2_{\Delta}$ by our choice of scale and rotation. As an example, consider the case where $n = 2$. Then, $L_1$ maps  $(1,0)$ to $\left( \frac{3}{2}, \frac{\sqrt{3}}{2} \right)$ and maps $\left(\frac{1}{2},\frac{\sqrt{3}}{2}\right)$ to $\left( 0, \sqrt{3} \right)$.  For a shape $S$ as shown in Figure~\ref{fig:scale-example-1}, $S' = L_1(S)$ is shown in Figure~\ref{fig:scale-example-1}, and the $2$-scaling of $S$ is shown in Figure~\ref{fig:scale-example-3}.

Secondly, to define the offset $n$-scaling of $S$ we let $L_2$ be the linear transformation of $\mathbb{R}^2$ which maps $(1,0)$ to $\left( \frac{3n-1}{2}, \frac{\sqrt{3}(n-1)}{2} \right)$ and maps $\left(\frac{1}{2},\frac{\sqrt{3}}{2}\right)$ to $\left( \frac{1}{2}, \frac{\sqrt{3}}{2}(2n-1) \right)$. Then, let $S^* = L_2(S)$.  Then the offset $n$-scaling of $S$ is the union over all $\vec{p}$ in $S^*$ of sets of points $Hex_n + \vec{p}= \{\vec{v}\in R^2 | \vec{v} = \vec{h} + \vec{p} \text{ for some } \vec{h}\in Hex_n \}$.  One can observe that the points of $S^*$ is a subset of $\Z^2_{\Delta}$ by our choice of scale and rotation. Again, consider the case where $n = 2$. Then, $L_1$ maps  $(1,0)$ to $\left(( \frac{5}{2}, \frac{\sqrt{3}}{2} \right)$ and maps $\left(\frac{1}{2},\frac{\sqrt{3}}{2}\right)$ to $\left( \frac{1}{2}, \frac{3\sqrt{3}}{2} \right)$. For a shape $S$ as shown in Figure~\ref{fig:scale-example-1}, $S^* = L_2(S)$ is shown in Figure~\ref{fig:offset-scale-example-2}, and the offset $2$-scaling of $S$ is depicted in Figure~\ref{fig:offset-scale-example-3}.


==> definitions-informal.tex <==
\section{The Oritatami Model}

%\todo{ED: I find $h$-interactions vs.\ bonds confusing. Why multiple terms? Does $h$ stand for something? If $h$ isn't a variable, it at least shouldn't be in math mode.} %agreed

In this section we give intuitive definitions related to the oritatami model. For more formal definitions see Section~\ref{sec:definitions-formal} The oritatami model of molecular folding is based on co-transcriptional folding where strands of RNA nucleotides fold to form complex structures during the process of transcription. Informally, one can think of an oritatami system (OS) as capturing the folding of an ever-elongating string of equally spaced \emph{beads} onto a triangular grid graph, which we call $\mathbb{T}$, into \emph{configurations}. We note that we choose the particular triangular grid graph whose vertices are a subset of $\mathbb{R}^2$ of equilateral triangles such that $\mathbb{T}$ contains $(0,0)$ and $(1,0)$ as vertices and an edge between $(0,0)$ and $(1,0)$. For the formal definition, see Section~\ref{sec:definitions-formal}.  Modeling folding on a triangular grid\footnote{as opposed to the $\Z^2$-lattice that defines the underlying structure of most tile assembly models such as the abstract Tile Assembly Model~\cite{Winf98}} permits greater variability in the how a structure may fold as well as greater variety in the types of interactions between beads as a point of a triangular grid can have up to 6 neighboring points. For this reason, the triangular grid seems more suitable to model the systems that produce complexes that result from cotranscriptional-like folding. See~\cite{Nubots, derakhshandeh2016universal} for models of self-organizing matter where fundamental components of the model also organize on a triangular grid. 

For a finite alphabet $\Sigma$, a bead is defined to be a point in $\mathbb{T}$ that is labeled with an element of $\Sigma$. Elements of $\Sigma$ are called \emph{bead types}. Pairs of beads may ``attract'' each other and whether or not one bead attracts another bead is given by a set of pairs of bead types called the \emph{rule set}. Note that the rule set defines a symmetric relation. A configuration captures the ``state'' of an OS and is defined to be a path of beads $R$ in pairwise distinct positions in $\mathbb{T}$, along with a set of pairs of beads in $R$ called the set of \emph{bonds} which specify an ``attraction'' between beads in $R$. We call the path of beads $R$ the \emph{routing} of the configuration. Therefore, a configuration is a routing together with a set of bonds. We say that a configuration is finite when the sequence of beads defining the configuration is finite. A \emph{valid} configuration is one in which each bonds between two beads, $b_1 = (p_1, w_1)$ and $b_2 = (p_1, w_1)$ say, is such that $(w_1, w_2)$ is in the rule set. 
%
%
Then, an \emph{oritatami system (OS)} is a $7$-tuple $\Xi = (\Sigma, w, \calH, \delta, \beta, \alpha, \sigma)$ where
\begin{itemize}
  \item $\Sigma$ is a set of bead types,
  \item $w \in \Sigma^* \cup \Sigma^\omega$ is a periodic sequence which we call the \emph{transcript} of $\Xi$,
  \item $\calH$ is a set of pairs of bead types called the \emph{rule set},
  \item $\delta \in \mathbb{N}$ is called the \emph{delay},
  \item $\beta \in \mathbb{N}$ is called the \emph{\extlen},
  \item $\alpha \in [1,6]$ is called the \emph{arity}, and
  \item $\sigma$ is a valid configuration which we call the \emph{seed}.
\end{itemize}
%
When talking about oritatami systems we will talk about the sequences of configurations that lead from the initial structure which we call the \emph{seed} all the way to the final product.  As we will see, in such a sequence, each set of possible consecutive configurations is completely determined by the previous configuration. 
%
Let $\Xi = (\Sigma, w, \calH, \delta, \beta, \alpha, \sigma)$ be an OS. The three parameters $\delta$, $\beta$, and $\alpha$ govern the folding process by determining how to use $w$ and $\calH$ to transition from one configuration to the next, and the seed configuration $\sigma$ serves as the initial configuration of $\Xi$. The parameters $\delta$, $\beta$, and $\alpha$ determine the transition from the seed $\sigma$ to another valid configuration, $C$ say, as follows. 

First, let $R$ be the routing defining $\sigma$ and let $H$ be the set of bonds for $\sigma$. Let $\calP$ be the set of all valid configurations with at most $\alpha$ bonds obtained by extending $R$ by up to $\delta$ beads, $b_1, b_2, \dots, b_{n}$, where $n\in \N$ and $n \leq \delta$, and  the label of bead $b_i$ is the $i$th bead type of $w$. We call configurations in $\calP$ \emph{elongations}. Note that the parameter $\alpha$ restricting the number of bonds allowable for a configuration here. Also note that by definition each configuration in $\calP$ has a set of bonds. Let $\calF$ be the set of configurations in $\calP$ with the greatest number of bonds. We call configurations in $\calF$ \emph{favorable elongations}. Then, let $C_\calF$ be some configuration in $\calF$, let $R_\calF$ be the routing of $C_\calF$, and let $H_\calF$ be the set of bonds of $C_\calF$. Note that $R_\calF$ is equal to $R$ extended by $n$ beads where $n\in \N$ and $n\leq \delta$ beads. 
%
Then, if $\beta \leq n$\footnote{Throughout this paper, $\beta$ is assumed to be $1$.}, let $R_C$ be the path of beads $R_\calF$ with $n-\beta$ beads removed and $R_\calF$ otherwise. The set of beads removed from $R_\calF$ to obtain $R_C$ is referred to as the set of \emph{nascent} beads of $R_\calF$ and the beads in $R_C$ that are not in $R$ are referred to as \emph{stabilized} beads of $R_\calF$. Moreover, let $H_C$ be the set of bonds obtained by removing all pairs of beads (i.e. bonds) such that at least one bead in the pair is a nascent bead. Then, $C$ is defined to be the configurations with routing $R_C$ and set of bonds $H_C$. We note that $C$ is a valid configuration since by definition $C_\calF$ is a valid configuration. Just as $C$ was obtain from $\sigma$, given any valid configuration, $C'$ say, we can similarly define the transition from $C'$ to a valid configuration $C''$. Such transitions define a step (or fold) in the self-assembly process of an OS. Moreover, this notion of transition gives rise to sequences of configurations which we call \emph{foldable sequences over $w$ from configuration $C'$ to $C''$} for the OS $\Xi$ where each configuration in the sequence except for the first (i.e. $C'$) is obtained from the previous by a single transition and the final configuration is $C''$.  Moreover, foldable sequence over $w$ may be infinite, starting from some configuration $C'$ and continuing indefinitely. In Section~\ref{sec:definitions-formal} we note that such an infinite sequence has a unique limiting infinite configuration called the \emph{result} of the foldable sequence. A configuration $C$ is \emph{foldable} (or ``self-assembles'' in $\Xi$) by the OS $\Xi$ if there is a foldable sequence over $w$ from $\sigma$ to $C$, and a \emph{terminal} configuration is one that is not properly contained in any other configuration. Then the set of  all \emph{foldable} configurations by an OS $\Xi$ is denoted by $\prodasm{\Xi}$, and the set of all terminal configurations of $\Xi$ is denoted by $\termasm{\Xi}$. When $|\termasm{\Xi}| = 1$, we say that $\Xi$ is \emph{deterministic}.

For an example of how to transition from one configuration to another, see Figure~\ref{fig:definitions-examples}.
%
\begin{figure}[ht]
\centering
    \begin{subfigure}[b]{1in}
	\centering
	\includegraphics[width=.7in]{images/definition-example0}
	\caption{}
    \label{fig:definition-example0}
    \end{subfigure}
\quad\quad
    \begin{subfigure}[b]{1in}
	\centering
	\includegraphics[width=1in]{images/definition-example1}
	\caption{}
    \label{fig:definition-example1}
    \end{subfigure}
\quad\quad
    \begin{subfigure}[b]{1in}
	\centering
	\includegraphics[width=1in]{images/definition-example2}
	\caption{}
	\label{fig:definition-example2}
    \end{subfigure}
\quad\quad
    \begin{subfigure}[b]{1in}
	\centering
	\includegraphics[width=1in]{images/definition-example4}
	\caption{}
	\label{fig:definition-example3}
    \end{subfigure}
\quad\quad
    \begin{subfigure}[b]{1in}
	\centering
	\includegraphics[width=1in]{images/definition-example3}
	\caption{}
	\label{fig:definition-example4}
    \end{subfigure}
    
	\caption{(a)-(e) An example of the dynamics of an oritatami system $\Xi$ with alphabet $\Sigma = \{a,b,c,d,e,f,g,h,i,j,k\}$. We assume that this system has transcript $w = abcdefghijk$, that $(d,f)$, $(b,d)$, and $(b,e)$ are in the rule set, and arity is $2$. (a) An example configuration, $\sigma$ say, in an OS. (b) An elongation of $\sigma$ by $3$ beads. Such an elongation would be considered when $\delta = 3$. (c) Another elongation of $\sigma$ by $3$ beads that has more bonds than the elongation shown in (b) and is therefore more favorable. In (d) and (e), assume that this is in fact a favorable elongation. Note that this configuration is considered for arity $2$ but would not be considered if arity was $1$. (d) If $\beta = 1$, the bead $d$ is a stabilized bead of the elongation shown in (c), while beads $e$ and $f$ are nascent. To obtain the another configuration from the configuration in (d), we consider the favorable elongations with $3$ beads with types $g$, $h$, and $i$. (e) If $\beta = 2$, $d$ and $e$ are both stabilized beads and $f$ is a nascent bead.}
	\label{fig:definitions-examples}
\end{figure}
%
%%
%\begin{wrapfigure}{r}{0.4\textwidth}
%\vspace{-40pt}
%  \begin{center}
%    \includegraphics[width=0.38\textwidth]{images/definition-config-example}
%  \end{center}
%  \caption{An example of a configuration in an OS.\vspace{-12pt}}
%  \label{fig:definition-config-example}
%\end{wrapfigure}
%%
%%
%Figure~\ref{fig:definition-config-example} gives an example of a configuration that is the result of a foldable sequence of configuration for the OS $\Xi$ with seed $\sigma$ shown as black beads in the figure. The alphabet $\Sigma$ of $\Xi$ is $\{a, b, c, d, e, f, g, h, i, j\}$ and the transcript $w$ is the infinite periodic sequence of $abcdefghi$ repeated indefinitely. The rule set $\calH$ is the symmetric closure of the set\footnote{The symmetric closure $S_c$ of a set of pairs of symbols $S$ is given by $S_c = \{(a,b) | (a,b)\in S$ or $(b,a)\in S\}$.} $\{(a,c),$ $(b,d),$ $(c,e),$ $(d,f),$ $(g,e),$ $(e,h),$ $(h,j),$ $(a,e),$ $(b,i)\}$. Moreover, $\delta = \beta = 1$ and $\alpha = 3$. Note that this configuration could not be the result of a foldable sequence if arity $\alpha$ is less than $3$ as $3$ bonds would not be allowed.
%
%\begin{figure}[htp]
%\centering
%\includegraphics[width=3.0in]{images/definition-config-example}
%\caption{An example of a configuration in an OS.}
%\label{fig:definition-config-example}
%\end{figure}
%

When self-assembling finite shapes in an oritatami systems, we consider the number of bead types called, \emph{bead complexity}, and the length of the transcript, called \emph{transcript complexity} as measures of complexity of an OS.

\subsection{Shapes and scaling}

We now give informal definitions that pertain to shapes. See Section~\ref{sec:shape-defs} for more formal definitions.

Denote the points in $\mathbb{R}^2$ that correspond to vertices of $\calT$ by $\Z^2_{\Delta}$.
A \emph{shape} $S$ is a set of connected points in $\Z^2_{\Delta}$. 
%
Given an OS system $\Xi$ and a shape $S$, we say that $\Xi$ \emph{folds} (or ``self-assembles'') $S$ if for any terminal configuration $C$ of $\Xi$, the set of points defined by the locations in $\Z^2_{\Delta}$ of beads of the routing $R$ of $C$ is equal to $S$. In other words, $\Xi$ folds $S$ if every terminal assembly of $\Xi$ contains a bead at a location if and only if this location is in $S$. As we will see, it is not always possible to fold a shape $S$. However, when $S$ is finite and connected, it is possible to fold a \emph{scaling} of $S$. As folding occurs in the triangular grid graph, there are multiple ways in which one could scale a shape. We define two such notions here. While these notions of scaling are similar, properties of these scaling methods make them useful for different purposes. In particular, the first method of scaling that we will define will help lead to an algorithm for finding a Hamiltonian cycle in a scaled shape that is scaled using this first method. Interestingly, a second method for scaling a shape is more useful when defining oritatami gadgets which fold a scaled version of a shape that is scaled using the second method for scaling. We now define these two notions of scaling compatible for shapes in the triangular grid graph. The two methods of scaling that we define are called the \emph{$n$-scaling} of $S$ and the \emph{offset $n$-scaling} of $S$. For both methods of scaling, we refer to $n$ as the \emph{scale factor}.

To define both of the methods of scaling a shape, we define two linear transformations of $\mathbb{R}^2$ (one for each scaling method). Intuitively, these linear transformations expand the distance between the points in $S$ equally by a specific amount and rotate these points so that all of the points of $S'$ belong to $\Z^2_{\Delta}$. We then obtain a scaling of $S$ by replacing a point $\vec{p}$ of $S'$ by points of a solid hexagon with side length $n$\footnote{More specifically, the hexagon of points in $\Z^2_{\Delta}$ equal to the set $\{ \vec{v} \in \Z^2_{\Delta}  |  \d(\vec{0}, \vec{v}) < n \}$.} translated so that the center of the hexagon is $\vec{p}$. Figure~\ref{fig:scale-example-shape} describes both scaling methods. The main difference between an $n$-scaling of a shape $S$ and an offset $n$-scaling of $S$ is that while the points of $S$ are represented by a solid hexagon of points, in an $n$-scaling, these hexagons of points overlap when representing two adjacent points in $S$ and in an offset $n$-scaling, these hexagons that represent points in $S$ are all disjoint. 

\begin{figure}[ht]
\centering
    \begin{subfigure}[b]{1in}
	\centering
	\includegraphics[width=1in]{images/scale-example-1}
	\caption{}
    \label{fig:scale-example-1}
    \end{subfigure}
\quad
    \begin{subfigure}[b]{1in}
	\centering
	\includegraphics[width=1in]{images/scale-example-2}
	\caption{}
    \label{fig:scale-example-2}
    \end{subfigure}
\quad
    \begin{subfigure}[b]{1in}
	\centering
	\includegraphics[width=1in]{images/scale-example-3}
	\caption{}
	\label{fig:scale-example-3}
    \end{subfigure} 
\quad
    \begin{subfigure}[b]{1in}
	\centering
	\includegraphics[width=1in]{images/offset-scale-example-2}
	\caption{}
    \label{fig:offset-scale-example-2}
    \end{subfigure}
\quad
    \begin{subfigure}[b]{1in}
	\centering
	\includegraphics[width=1in]{images/offset-scale-example-3}
	\caption{}
	\label{fig:offset-scale-example-3}
    \end{subfigure}    
	\caption{(a) An example shape $S$, (b) a depiction of the points of $S$ scaled and rotated points by the linear transformation $L_1$, (c) the $2$-scaling of $S$, (d) a depiction of the points of $S$ scaled and rotated points by the linear transformation $L_2$, (e) the offset $2$-scaling of $S$}
	\label{fig:scale-example-shape}
\end{figure}




\subsubsection{Weakly connected shapes}

The self-assembly of shapes in oritatami systems is fundamentally different from the self-assembly of shapes in tile assembly systems due to the fact that every configuration in an OS has a routing that is a path of beads. To illustrate this difference, we define a property for shapes called \emph{weakly connected} that is satisfied if there exists a finite subset of points $K$ in $S$ such that $S\setminus K$ contains at least two infinite sets $S_1$ and $S_2$ such that for any two points $p$ and $q$ with $p$ in $S_1$ and $q$ in $S_2$, $p$ and $q$ are not path connected.  As a preliminary result, we have the following theorem. The proof of this theorem can be found in Section~\ref{sec:branching-shapes}.

\begin{theorem}\label{thm:infinite-shapes-short}
Let $S$ be a weakly connected shape. Then for any OS $\Xi$, $S$ is not foldable in $\Xi$.
\end{theorem}

Note that since the $n$-scaling of $S$ and the offset $n$-scaling of $S$ are both weakly connected, a corollary of Theorem~\ref{thm:infinite-shapes-short} is that for all $n\in \N$, if $S$ be a weakly connected shape, then the $n$-scaling of $S$ and the offset $n$-scaling of $S$ are not foldable by any OS.


==> infinite-shapes.tex <==
\section{Infinite Shapes With Finite Cut Are Not Foldable}\label{sec:branching-shapes}

In the abstract Tile Assembly Model as well as other tile assembly models, tiles may attach at many different locations resulting in assembly sequences where assemblies branch and extend indefinitely in one or more directions. In contrast, an infinite configuration in an oritatami systems is defined by a routing which is a one-way infinite path of beads in $\Tlat$. Due to this fact, there are many infinite shapes which do not self-assemble in any OS. Theorem~\ref{thm:infinite-shapes} formalizes this statement. Before we consider this theorem, we give a few definitions. Let $S\subseteq \Z^2_{\Delta}$ be a shape. 
%
%
%
Let $S$ be an infinite connected shape. We say that $S$ has a \emph{finite cut} if there is a finite subset of points $K$ in $S$ such that $S\setminus K$ contains at least two infinite connected components $S_1$ and $S_2$. 

The following theorem states a fundamental restriction on the types of infinite shapes that are foldable by an OS that is due to the fact that every configuration in an OS has a routing that is a path of beads. 

\begin{theorem}\label{thm:infinite-shapes}
Let $S$ be an infinite shape having a finite cut. Then for any OS $\TMO$, $S$ is not foldable in $\TMO$.
\end{theorem}

\begin{proof}
Let $K$ be a finite subset of $S$ such that $S\setminus K$ contains two infinite connected components $S_1$ and $S_2$. For the sake of contradiction, suppose that $\TMO$ is an OS and $S$ is foldable in $\TMO$. 
%
As $S$ is foldable in $\TMO$ by assumption, there must exist a foldable sequence, $\vec{C} = \{C_i\}_{i=1}^\infty$ say, with result $S$ and $C_i$ a valid foldable configuration in $\TMO$. Note that we can find a sequence of points in $S$ $\{q_i\}_{i=1}^{|K|+1}$ such that the following properties hold. (1) $q_i$ is in $S_1$ for $i$ odd and $q_i$ is in $S_2$ for $i$ even, and (2) for some $j\in \N$, $q_i$ is a location for a bead in $C_j$ but not a bead in $C_{j-1}$. Then, by Property (2), the routing of $C_j$ must contain a path from a bead at location $q_{i-1}$ to a bead at location $q_i$ as a subpath for each $i$ between $1$ and $|K|+1$ inclusive. By Property (2), this subpath must must contain a point in $K$ for otherwise, we arrive at a contradict of the assumption that $S$ is weakly connect. Moreover, one can show that $C_j$ must contain beads at $i$ many distinct points in $K$. Therefore, for $i = |K|+1$, such a configuration $C_j$ contains $|K|+1$ distinct points of $K$. Hence we arrive at a contradiction. Therefore, $S$ is not foldable in $\TMO$.
\end{proof}

As any scaling of an infinite shape with a finite cut has a finite cut, we get the following corollary:

\begin{corollary}
For every infinite shape $S$ having a finite cut, every scaling $\Lambda$, there is no oritatami system that folds $\Lambda(S)$.
\end{corollary}


==> introduction.tex <==
\section{Introduction}

Transcription is the process in which an RNA polymerase enzyme (colored in orange in Figure~\ref{fig:rna_origami}) synthesizes the temporal copy (blue) of a gene (gray spiral) out of  ribonucleotides of four types {\tt A}, {\tt C}, {\tt G}, and {\tt U}.
The copied sequence is called the \textit{transcript}.
%
\input{fig-RNA-origami.tex}
%
The transcript folds \textit{cotranscriptionally}, that is, it starts folding upon itself into intricate tertiary structures immediately after it emerges from the polymerase, as illustrated in the cotranscriptional folding of RNA tile structure 
 out of an artificial gene engineered by Geary, Rothemund, and Andersen \cite{GeRoAn2014} (see Figure~\ref{fig:rna_origami}).
The RNA tile is provided with a kissing loop (KL) structure, which yields a $120^{\circ}$ bend, at its four corners, and sets of six copies of it self-assemble into hexagons and further into a hexagonal lattice.
\emph{Structure} is almost synonymous to \emph{function} for RNA complexes since they are highly correlated, as exemplified by various natural and artificial RNAs \cite{MolBiolRNA}.
%by naturally occurring RNAs including transfer RNA and ribosomal RNA, as well as by artificial RNAs like the RNA tile \cite{MolBiolRNA}.
Cotranscriptional folding plays significant roles in determining the structure (and hence function) of RNAs. %and there are many examples illustrating the importance of cotranscriptional folding in determining the structure of RNAs.
%To give a few examples, introns along a transcript cotranscriptionally fold into a loop recognizable by spliceosome and get excised \cite{MerkhoferHuJohnson2014}, and 
As an example, riboswitches make a decision on gene expression by folding cotranscriptionally into one of two mutually exclusive structures: an intrinsic terminator hairpin and a pseudoknot, as a function of specific ligand concentration \cite{WaStYuLiLu2016}.
What is folded is affected by various environmental factors including transcription rate.
Polymerases have their own transcription rate: e.g., bacteriophage 3ms/nucleotide (nt) and eukaryote 200ms/nt \cite{Isambert2009} (less energy would be dissipated at slower transcription \cite{FeynmanLecComp}).
Changing the natural transcription rate, by adjusting, e.g., NTP concentration \cite{ReWiRaScRiSt1999}, can impair cotranscriptional processes \cite{ChaoKanChao1995, LeMaReNi1993} (note that polymerase pausing can also facilitate efficient folding \cite{WongSosnickPan2007} but it is rather a matter of gene design).
Given a target structure, it is hence necessary to know not only what to fold but at what rate to fold, that is, to know when to fold `em.

The primary goal of both natural and artificial self-assembling systems is to form predictable structures, i.e. shapes grown from precisely placed components, because the form of the products is what yields their functions.
The route of transcript of the RNA tile (Figure~\ref{fig:rna_origami}) was not given \textit{a priori}, but the architects tried various Hamiltonian paths through the rectangle (shape) as a route and checked whether the transcript folds cotranscriptionally along them so as to yield the intended functions, that is, KL's at the four corners.
This motivates the study of shape self-assembly problems using a novel mathematical model of cotranscriptional folding called \textit{oritatami system} (abbreviated as OS) \cite{GeMeScSe2016}. 
%As this is ultimately the primary goal in self-assembly, here we focus on this class of problems.
Mathematical models have proven useful in developing an understanding of how shapes may self-assemble, % and self-assembling finite shapes is one of the fundamental goals of theoretical modeling of systems capable of self-assembly.
e.g. in tile-based self-assembly~\cite{RNAPods,DDFIRSS07,SolWin07} as well as other models of programmable matter~\cite{derakhshandeh2016universal, Nubots}.
%Often the goal in self-assembling a shape is to do so while minimizing the complexity of the required system. For example, in the abstract Tile Assembly Model, the measurement of complexity is the number of distinct types of tiles, and indeed, in~\cite{SolWin07}, the number of tile types required to self-assemble finite shapes at some scale factor is shown to be bounded above and below by the Kolmogorov complexity of the shape. 
Just as these models set out to capture processes of self-assembly by aggregation, the oritatami model sets out to capture the process of self-assembly by cotranscriptional folding.

%An oritatami system (abbreviated as OS) is a novel mathematical model of cotranscriptional folding \cite{GeMeScSe2016}.It abstracts an RNA tertiary structure as a triple of 1) a sequence of abstract molecules (of finite types) called \emph{bead types}, 2) a directed path over a triangular lattice of \emph{beads} (i.e. a location/bead type pair), and 3) a set of pairs of adjacent beads that are considered to interact with each other via hydrogen bonds. Such a triple is called a \textit{configuration}. An abstraction of the RNA tile~\cite{GeRoAn2014} as a configuration is shown in Figure~\ref{fig:rna_origami} (Right). In the figure, each bead (represented as a dot) abstractly represents a sequence of 3-4 nucleotides, whose type is not stated explicitly but retrievable from the transcript's sequence of the tile (available in \cite{GeRoAn2014}); moreover, the interactions (or bonds) between pairs of beads are represented by dashed lines. An OS is provided with a finite alphabet $\Sigma$ of bead types, a sequence $w$ of beads over $\Sigma$ called its \textit{transcript}, and a rule set $\mathcal{H}$, which specifies between which types of beads interactions are allowed. The OS cotranscriptionally folds its transcript $w$, beginning from its initial configuration (\textit{seed}), over the triangular lattice by stabilizing beads of $w$ from the beginning one by one.\footnote{An addition parameter $\beta$ called \emph{\extlen} can be specified so that beads stabilize $\beta$ by $\beta$ instead of one by one.} Two parameters of OS govern the bead stabilization: \textit{arity} and \textit{delay}; arity models valence (number of bonds per bead). Delay models the transcription rate in the sense that the system stabilizes the next bead in such a way that the sequence of the next bead and the $\delta-1$ succeeding beads is folded so as to form as many bonds as possible; hence, delay~1 models slowest possible transcription.

The oritatami system abstracts an RNA structure as a triple of 1) a sequence $u$ of abstract molecules (of finite types) called \textit{bead types}, 2) a directed path (routing) $r$ over the triangular lattice $\mathbb{T}$, and 3) a set $H$ of pairs of adjacent beads that are considered to interact with each other via hydrogen bonds. 
See Figure~\ref{fig:rna_origami} for such an abstraction of RNA tile. 
Upon its initial "seed" structure $\sigma$, a delay-$\delta$ oritatami system folds its transcript $w$, a sequence of bead types, over the triangular lattice $\mathbb{T}$ cotranscriptionally at the transcription rate $\delta$.
That is, it stabilizes the first bead $w[1]$ of the transcript so as for the sequence of it and its consecutive $\delta-1$ beads, i.e., $w[1..\delta]$ to form as many bonds as possible, and once $w[1]$ is stabilized, the bead $w[\delta+1]$ is transcribed for the local optimization of the sequence $w[2..\delta+1]$ to stabilize $w[2]$, and so on. 
The delay parameter thus models the transcription rate. 
The other parameter \textit{arity} imposes the maximum number of bonds that one bead can form. 

Using this model, researchers have mainly explored the computational power of cotranscriptional folding (see recent surveys \cite{RogersSeki2017, Seki2017}).
%Geary et al.~proved that at delay~3, deterministic OS's are efficiently Turing-universal using 542 bead types \cite{GeMeScSe2017} (some of these bead types might be saved by heuristic algorithms by Han and Kim \cite{HanKim2017}).See recent surveys \cite{RogersSeki2017, Seki2017} on oritatami for other results.
In contrast, little has been done on self-assembly of shapes.
Elonen informally sketched how an OS can fold a transcript all of whose beads are of pairwise-distinct types (hardcodable transcript) into a finite shape with Hamiltonian path \cite{Elonen2016}. 
Masuda et al.~implemented an OS that folds its periodic transcript into a finite portion of the Heighway dragon fractal \cite{MasudaSekiUbukata}.
Rogers and Seki proposed a notion of simulation of an OS by another such that the simulator must follow the same route as the simulated \cite{RogersSeki2017}.
This notion is however too restrictive to address shape self-assembly problems; the simulator should be entitled to its freedom of choice in routing of transcript.

We initiate a systematic study of shape self-assembly by oritatami system. 
By definition, a shape without Hamiltonian path cannot be self-assembled by any OS. 
This signifies the scaling-up in this study; we consider three scaling-up schemes in this paper: \scaling An, \scaling Bn, and \scaling Cn (see Fig~\ref{fig:def:upscaling:ABC}). 
For $n \ge 3$ and each of these scaling-up schemes, we propose an algorithm to generate a delay-1 OS over a universal 114 bead types and rule set that folds into the $n$-scaling of a given shape $S$ (Theorems~\ref{thm:scaling:algo:universal:bead:type}, \ref{thm:scaling:algo:routing:Bn}). 
This algorithm is incremental; it can modify the OS it produced for $S$ when a new point is added to $S$ just by local re-routing. 
Thus, the algorithm runs in linear time. 
This algorithm is augmented with our construction of an OS that allows to fold the \scaling A2, \scaling B2, and \scaling C2 of an arbitrary finite shape as long as the delay can be set arbitrarily long (Theorem~\ref{thm:hard-coded}). 
This algorithm requires arity higher than 1. 
In fact, setting arity to 1 bounds the size of determinisitcally-foldable shapes at delay 1 linearly by the size of the seed (Theorem~\ref{thm:d1a1_det_finiteness_short}). 
This implies computational weakness, which might explain natural transcription rate being set not so slow even at the cost of higher energy consumption. 
The scaling is not universal; indeed, we prove that an infinite shape of finite cut cannot be folded by any OS (Theorem~\ref{thm:infinite-shapes-short}). 

Lastly, we analyze the OS' capability of self-assembling shapes with respect to delay. 
Scaling has not proved useful yet for self-assembling infinite shapes by OS, as noted above. 
For delay $\delta > 2$, we construct an infinite shape $S_\delta$ that can be folded by an OS at delay $\delta$ but cannot be folded by any OS at shorter delay (Theorem~\ref{thm:small-delay-weak}). 

%We first provide an enhanced set of definitions for the OS which are intended to make the model both more understandable and easier to work within by providing tools useful for proving both positive and negative results.
%We prove that there is a single set of bead types $\Sigma$ and rule set $\calH$ such that given an arbitrary finite shape $S$ (i.e. a set of connected points in the triangular grid) there is an OS $\Xi$ with bead types $\Sigma$ and rule set $\calH$ that folds a scaled (by a constant factor) version of shape $S$. Moreover, $\Xi$ has a seed configuration of size $4$, delay $1$ and arity $4$. This result is given in Theorem~\ref{thm:finite-shapes}. To prove this theorem, we give a polynomial time algorithm that takes an arbitrary finite shape $S$ as input and outputs the OS $\Xi$.


%Our results

%\begin{enumerate}
%    \item At scale factor 1:
%    \begin{enumerate}
%        \item There exists shape $S$ such that $|S| < \infty$, but no oritatami system can self-assemble $S$
%	    \item $\forall \delta > 1$, there exists a shape $S_{\delta}$ such that there exists an oritatami system $O_{\delta}$ which can self-assemble $S_{\delta}$ at delay factor $\delta$, but no oritatami system exists which can self-assemble $S_{\delta}$ at delay factor $\delta' < \delta$.
%	    Old text: We study the effect that different delay factors have on the possibility of folding shapes. In particular, we show (Theorem~\ref{thm:small-delay-weak}) that for any delay factor $\delta > 2$, there exists an infinite shape $S$\footnote{We consider folding infinite shapes, but the result that we show applies to OS's with a fixed constant seed size.} such that $S$ folds in an OS with delay factor $\delta$, but does not fold in any OS with delay factor less than $\delta$, which provides the first direct proof of the differing theoretical powers of varying speeds of transcription.
%    \end{enumerate}

%\item At any scale factor:
%    \begin{enumerate}
%        \item There exist infinite shapes that cannot be made at any delay factor:  we give a simple condition for a shape called \emph{weakly connected} and show that no OS can fold a weakly connected shape (Theorem~\ref{thm:infinite-shapes-short}).
%    \end{enumerate}
%
%\item At scale factors 2.0, 2.0+, and 2.5:
%    \begin{enumerate}
%	    \item with no restriction on delay factor, all finite shapes can be made
	    %\item at every delay factor, there exists a finite shape which cannot be made
%	\end{enumerate}
%\item At all scale factors 3.0 or greater:
%    \begin{enumerate}
%	    \item finite shape can be made at a constant delay factor
%	\end{enumerate}
%\item Lastly, we prove that setting both delay and arity to 1 bounds the size of deterministically-foldable shapes linearly by the size of seed (Theorem~\ref{thm:d1a1_det_finiteness_short}), implying computational weakness \cite{jLSAT1, Ibarra1978}, which is in sharp contrast with the efficient Turing universality at delay~3.
%This weakness might explain natural transcription rate being set not so slow even at the cost of higher energy dissipation.
%\end{enumerate}


%The main results/contributions of this paper are the following:
%\begin{enumerate}
%%    \item We provide an enhanced set of definitions for the Oritatami model which are intended to make the model both more understandable and easier to work within by providing tools useful for proving both positive and negative results.
%%    \item For a general finite shape, it is NP-complete to determine whether there exists an Oritatami system which self-assembles it, because it is NP-complete to determine if there is a path through it.
%    \item There exists a constant scale factor such that any finite shape can be scaled and self-assembled, and an efficient algorithm to output the necessary Oritatami system.  We provide such an algorithm and prove its correctness.
%    \item For each delay factor $\delta > 1$, there exists a shape $S$ such that $S$ can self-assemble by an Oritatami system at delay factor $\delta$, but no Oritatami system with delay factor $\delta' < \delta$ exists in which $S$ self-assembles.
%    \item Shin has a result stating the impossibility of systems with delay factor $1$ to be directed and self-assemble infinite shapes, I believe.  I'll let him correct this and add the necessary details...
%\end{enumerate}

%\todoi{MJP: We need to be consistent with capitalization.  I've been capitalizing Oritatami, but I don't think others have been.}
%\jghtodoi{I with capitalizing Oritatami, but don't care either way.}



==> no-long-lines-at-scale-1.tex <==
\subsubsection{No long lines}

\newcommand{\linelen}{%
\ensuremath{6\delta^2 + 2\delta}
}

\newcommand{\bondcount}[1]{%
\ensuremath{\#bonds(#1)}
}

We first consider OS's which fold lines. That is, we consider OS's for which any terminal configuration is either a finite or infinite set of colinear points. The following lemma shows that the length of the line which is foldable by such an OS is bounded by a value which only depends on the delay factor of the OS. [JGH: TODO: use notation $\dom{C}$ for the set of bead locations of $C$ throughout this section.]

\begin{lemma}\label{lem:no-long-lines}
Let $\Xi = (\Sigma, \omega, \calH, \delta, \beta, \alpha, \sigma)$ is an OS such that 
\begin{enumerate}
    \item the set of bead locations for beads in $\sigma$ is a set of  colinear points,
    \item $|\sigma| = \delta + 1$,
    \item $\beta = 1$, and
    \item for any terminal configuration $C$ of $\Xi$, the set of bead locations for beads in $C$ is a set of colinear points.  
\end{enumerate}

Then, for any terminal configuration $C$ of $\Xi$, $|C| < \linelen$. 
\end{lemma}

\begin{proof}
Suppose that $\Xi = (\Sigma, \omega, \calH, \delta, \beta, \alpha, \sigma)$ be an OS such that 
\begin{enumerate}
    \item the set of bead locations for beads in $\sigma$ is a set of colinear points,
    \item $|\sigma| = \delta + 1$,
    \item $\beta = 1$, and
    \item for any terminal configuration $C$ of $\Xi$, the set of bead locations for beads in $C$ is a set of colinear points.  
\end{enumerate}

For the sake of contradiction, suppose that there exists a terminal configuration $C$ of $\Xi$, $|C| \geq \linelen$. 

We now introduce a bit of notation. Let $C_1 = \sigma$ and let $\langle C_i \rangle_{i=1}^{\linelen}$ be a foldable sequence over $\omega$ from $C_1$ to $C_{\linelen}$. Note that the set of bead locations of beads in $C_{\linelen}$ consists of $\linelen + |\sigma|$ colinear points. 

For $i\in \N$ such that $1\leq i \leq \linelen$, let $\mathcal{P}_i$ be the set of elongations of $C_i$, let $\mathcal{F_i}$ be the set of favorable configurations in $\mathcal{P}_i$, and let $b_{i+1}$ denote the bead in $C_{i+1}$ that is not in $C_{i}$. Moreover, we denote the number of bonds in $C_i$ by $\bondcount{C_i}$.


We now prove three claims which will help show Lemma~\ref{lem:no-long-lines}.

\begin{claim}\label{clm:lines0}
$\forall i \in \N$, let $f_i$ be an arbitrary configuration in $\mathcal{F}_i$. Then, $\bondcount{f_i} \leq 6\delta$. 
\end{claim}

\begin{proof}
Note that as the beads of $C_i$ are colinear, $\bondcount{C_i} = 0$. Hence the most bonds that can form between beads of any elongation of $\bondcount{C_i}$ by $\delta$ beads is $6\delta$. Thus, $\bondcount{f_i} \leq 6\delta$.
\end{proof}

\begin{claim}\label{clm:lines1}
$\forall i \in \N$ such that $1\leq i \leq \linelen$, let $f_i$ be an arbitrary configuration in $\mathcal{F}_i$. Then, $\bondcount{f_i} \geq 1$. 
\end{claim}

\begin{proof}
To prove Claim~\ref{clm:lines1} we note that if $\bondcount{f_i} = 0$ for some $i$, then any elongation of $C_i$ is favorable, including those elongations where the stabilized bead is not colinear with the beads of $C_i$. 
\end{proof}


\begin{claim}\label{clm:lines2}
$\forall i \in \N$ such that $1\leq i \leq \linelen$, let $f_i$ and $f_{i+1}$ be arbitrary configurations in $\mathcal{F}_i$ and $\mathcal{F}_{i+1}$ respectively. Then, $\bondcount{f_{i+1}} \geq \bondcount{f_{i}}$. 
\end{claim}

\begin{proof}
For the sake of contradiction, suppose that there exists $i \in \N$ such that $1\leq i \leq \linelen$ and for $f_i$ and $f_{i+1}$ configurations in $\mathcal{F}_i$ and $\mathcal{F}_{i+1}$ respectively, $\bondcount{f_{i+1}} < \bondcount{f_{i}}$. In this case, note that $\bondcount{f_{i}}$ is more favorable that $\bondcount{f_{i+1}}$, contradicting the fact that $\bondcount{f_{i+1}}\in \mathcal{F}_i$.
\end{proof}


\begin{claim}\label{clm:lines3}
$\forall i, j \in \N$ such that $1 \leq i, j \leq \linelen$, let $f_i$ and $f_{j}$ be arbitrary configurations in $\mathcal{F}_i$ and $\mathcal{F}_{j}$ respectively. Then, if $|i - j| > \delta$, $\bondcount{f_{j}} > \bondcount{f_{i}}$. 
\end{claim}

\begin{proof}
For some $i, j\in \N$ such that $|i - j| > \delta$, let $f_i$ and $f_{j}$ be arbitrary configurations in $\mathcal{F}_i$ and $\mathcal{F}_{j}$ respectively. Then, since $i\neq j$, without loss of generality, assume that $i < j$. By Claim~\ref{clm:lines2}, $\bondcount{f_{j}} \geq \bondcount{f_{i}}$. For the sake of contradiction, assume that $\bondcount{f_{j}} = \bondcount{f_{i}}$.

Note that $|f_i| = |\sigma| + i - 1 + \delta = 2\delta + i$.
By Claim~\ref{clm:lines1}, $\bondcount{f_i} > 0$. Therefore the $2\delta + i$ beads of $f_i$ cannot be colinear; otherwise, $\bondcount{f_i} = 0$. It follows from $\bondcount{f_{j}} = \bondcount{f_{i}}$ and the fact that $i+\delta < j$ that
$\forall k \in \N$ such that $i< k \leq i + \delta$, $\bondcount{f_k} = \bondcount{f_i}$. Therefore, $f_i\in \mathcal{F}_k$ for all $k$. $f_i$ is a foldable configuration of $\Xi$. Hence we arrive at a contradiction as the beads of $f_i$ are not colinear, yet we are under the assume that the beads of any foldable configuration of $\Xi$ are colinear. Therefore, Claim~\ref{clm:lines3} holds.
\end{proof}


Finally, we note that for $n = 6\delta + 2$, by Claim~\ref{clm:lines3}, for arbitrary choices of favorable configurations $f_i \in \mathcal{F}_i$ such that $i\in \{\delta, 2\delta, \dots, n\delta \}$, $\bondcount{f_{i-1}} > \bondcount{f_{i}}$. Hence, $\bondcount{f_{i}} \geq n = 6\delta + 2$. However, by Claim~\ref{clm:lines0}, $\bondcount{f_{i}} \leq 6\delta$. Therefore, we arrive at a contradiction, and Lemma~\ref{lem:no-long-lines} holds.
\end{proof}

%[JGH: generalize for all choices of $\beta$. This is straightforward.]


% \begin{figure}[htb]
% \centering
% \includegraphics[width=0.7\linewidth]{images/no-long-lines-intuition-1.pdf}
% \caption{Example where $\delta = 7$. Configuration extending from a line of length $\delta$ shown in red. $b_1$ is the first black bead from the left.}\label{fig:no-long-lines-1}
% \end{figure}

% \begin{figure}[htb]
% \centering
% \includegraphics[width=\linewidth]{images/no-long-lines-intuition-2.pdf}
% \caption{$\delta = 7$. Configuration extending from a line of length $\delta$ shown in red. $b_1$ is the first black bead from the left.}\label{fig:no-long-lines-2}
% \end{figure}


% \subsubsection{No long lines of subshapes of convex shapes connected by a single bead [JGH: change section title.]}

% Now we generalize this result to a line of lozenges and other shapes.  We will first consider ``lines of lozenges'', starting with the definition of such a shape. 

% Let \[S_0 =\left\{ \left(0,0\right), \left(\frac{1}{2}, \frac{\sqrt{3}}{2}\right), \left(1, 0\right), \left(\frac{3}{2}, \frac{\sqrt{3}}{2}\right)\right\}\text{, and for $d\in \N$, let }\]
% \[V_d = \left\{ \left(\frac{3n}{2}, \frac{3\sqrt{3}}{2} \right) \Bigg|\  n\in \N,\, 0\leq n \leq d \right\}\]

% For $d\in \N$, the ``line of lozenges'' of length $d$ is defined as the set $S_d = S_0 + V_d$. [JGH: define the sum of two sets of vectors to be the usual pairwise sum of vectors in each set]

% We now consider OS's which fold lines of lozenges. The following lemma shows that the length of the line of lozenges which is foldable by such an OS is bound by a value which only depends on the delay factor of the OS.

% \begin{lemma}\label{lem:no-long-lozenge-lines}
% Let $\Xi = (\Sigma, \omega, \calH, \delta, \beta, \alpha, \sigma)$ be an OS such that 
% \begin{enumerate}
%     \item $\dom{\sigma} = S_{\delta}$,
%     \item $\beta = 1$, and
%     \item for any terminal configuration $C$ of $\Xi$, there exists $d\in \N$ such that $\dom{C}$ is equal to $S_d$.  
% \end{enumerate}

% Then, for any terminal configuration $C$ of $\Xi$ such that $\dom{C} = S_d$, $d < \linelen$. 
% \end{lemma}

% \begin{proof}

% [JGH: the proof here is analogous to the proof of Lemma~\ref{lem:no-long-lozenge-lines}]

% Suppose that $\Xi = (\Sigma, \omega, \calH, \delta, \beta, \alpha, \sigma)$ is an OS such that 
% \begin{enumerate}
%     \item $\dom{\sigma} = S_{\delta}$,
%     \item $\beta = 1$, and
%     \item for any terminal configuration $C$ of $\Xi$, there exists $d\in\N$ such that $\dom{C} = S_d$.  
% \end{enumerate}

% For the sake of contradiction, suppose that there exists a terminal configuration $C$ of $\Xi$ such that $\dom{C} = S_d$, and $d \geq \linelen$. Note that there must be a configuration, which we denote by $C_{\linelen}$, that is foldable in $\Xi$ such that $\dom{C_{\linelen}} = S_d$. 


% [JGH: TODO: check notation and indices in the following]
% Let $D_1 = \sigma$ and let $\langle D_i \rangle_{i=1}^{3(\linelen) + 1}$ be a foldable sequence over $\omega$ from $D_1$ to $D_{3(\linelen) + 1}$ such that $\dom{C_{3(\linelen) + 1}} = S_{\linelen}$. Informally, $\langle D_i \rangle_{i=1}^{3*\linelen + 1}$ is the foldable sequence where we consider one bead added at a time. 
% %
% Let $C_0 = \sigma$ and let $\langle C_i \rangle_{i=0}^{\linelen}$ be a foldable sequence over $\omega$ from $C_0$ to $C_{\linelen}$ such that for any $i$ such that $1 \leq i \leq \linelen$,  $\dom{C_i} = S_i$. $\langle C_i \rangle_{i=0}^{\linelen}$ is the sequence of foldable configurations where one lozenge is added to obtain each consecutive configuration. Note that $C_i = D_{3i + 1}$. 


% For $i\in \N$ such that $1\leq i \leq \linelen$, let $\mathcal{P}_i$ be the set of elongations of $C_i$, let $\mathcal{F_i}$ be the set of favorable configurations in $\mathcal{P}_i$, and let $b_{i+1}$ denote the bead in $C_{i+1}$ that is not in $C_{i}$. Moreover, we denote the number of bonds in $C_i$ by $\bondcount{C_i}$.


% We now prove three claims which will help show Lemma~\ref{lem:no-long-lozenge-lines}. [JGH: these claims are a work in progress. ]

% \begin{claim}\label{clm:lozenge-lines0}
% $\forall i \in \N$ such that $2\leq i \leq \linelen$, $\bondcount{C_i} \leq \bondcount{\sigma} + 2i$. 
% \end{claim}

% \begin{proof}
% [JGH: TODO]
% \end{proof}

% \begin{claim}\label{clm:lozenge-lines1}
% $\forall i \in \N$, let $f_i$ be an arbitrary configuration in $\mathcal{F}_i$. Then, $\bondcount{f_i} \leq \bondcount{C_i} + 6\delta$. 
% \end{claim}

% \begin{proof}
% [JGH: TODO]
% \end{proof}

% \begin{claim}\label{clm:lozenge-lines2}
% $\forall i \in \N$ such that $1\leq i \leq \linelen$, let $f_i$ be an arbitrary configuration in $\mathcal{F}_i$. Then, $\bondcount{f_i} \geq \bondcount{D_{3i+1 + \delta}}$. 
% \end{claim}

% \begin{proof}
% [JGH: TODO]
% \end{proof}


% \begin{claim}\label{clm:lozenge-lines3}
% $\forall i \in \N$ such that $1\leq i \leq \linelen$, let $f_i$ and $f_{i+1}$ be arbitrary configurations in $\mathcal{F}_i$ and $\mathcal{F}_{i+1}$ respectively. Then, $\bondcount{f_{i+1}} \geq \bondcount{f_{i}}$. 
% \end{claim}

% \begin{proof}
% [JGH: TODO]
% \end{proof}


% \begin{claim}\label{clm:lozenge-lines4}
% $\forall i, j \in \N$ such that $1 \leq i, j \leq \linelen$, let $f_i$ and $f_{j}$ be arbitrary configurations in $\mathcal{F}_i$ and $\mathcal{F}_{j}$ respectively. Then, if $|i - j| > \delta$, $\bondcount{f_{j}} > \bondcount{f_{i}}$. 
% \end{claim}

% \begin{proof}
% [JGH: TODO]
% \end{proof}


% \end{proof}

% \begin{figure}[htb]
% \centering
% \includegraphics[width=\linewidth]{images/impossible-infinite.pdf}
% \caption{In this shape, the beads forming a horizontal line extend indefinitely to the right, and lines of increasing length branch from this horizontal line. For any OS with delay factor $\delta$, an infinite number of these ``branches'' must be of length greater than $6\delta^2 + 3\delta$.}\label{fig:impossible-infinite}
% \end{figure}

